EM^2Mem: Event-Centric Multimodal Memory for Large Language Models

Multimodal memory offers a scalable interface for long-video question answering, but existing methods often retrieve captions, frames, transcripts, summaries, or graph facts as isolated fragments. Although searchable, such fragments are not generation-ready: language models must reconstruct cross-modal and temporal alignments at inference time, when context is limited and attribution is difficult. We propose EM^2Mem, an event-centric multimodal memory framework that binds heterogeneous evidence to event anchors during memory construction. Each event-indexed memory cell aligns multimodal records, temporal context, graph-linked relations, semantic facts, and provenance, enabling compact evidence readout over grounded multimodal events rather than modality-specific fragments. Across three long-video QA benchmarks, EM^2Mem improves average accuracy over the strongest memory baseline by 2.0, 2.4, and 3.7 points, improves strict event-level Top-5 evidence recall by 7.0 points, and reduces per-query latency by 4.67 times and total inference tokens by 63.66% (The code will be integrated into https://github.com/zjunlp/LightMem).

==> tables/amortized_break_even_table.tex <==
\begin{table}[!tb]
\centering
\footnotesize
\setlength{\tabcolsep}{3.8pt}
\renewcommand{\arraystretch}{0.96}
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lrr@{}}
\toprule
\textbf{Criterion} 
& \textbf{Per-query saving} 
& \textbf{Break-even queries} \\
\midrule
Serial latency amortization
& 360.79s / query
& 28.6 \; ($\approx$29) \\
Practical evaluation throughput
& 446.73s / query
& 23.1 \; ($\approx$24) \\
Token-count amortization
& 53.52K tokens / query
& 535.9 \; ($\approx$536) \\
\bottomrule
\end{tabular*}
\caption{
Break-even analysis for amortizing the additional memory construction overhead of EM\textsuperscript{2}Mem.
The wall-clock break-even point is computed from the extra construction time of EM\textsuperscript{2}Mem over WorldMM, i.e., 10,314s.
Serial latency amortization uses the average per-query latency difference, 459.00s $-$ 98.21s.
Practical throughput amortization uses the measured end-to-end inference wall-clock time over the EgoLifeQA evaluation set.
Token-count amortization uses the additional construction token cost of EM\textsuperscript{2}Mem, 28.68M tokens, and the per-query inference token saving estimated from EgoLifeQA.
}
\label{tab:amortization-analysis}
\end{table}
